Unary Versus Binary Two-Way Automata

If L is a unary language, then its binary coded version bin(L) is a binary language containing all binary strings representing any 0^x in L. It is known that if a unary language L is regular and can be recognized by a minimal one-way deterministic finite automaton (1DFA) with n states, then its binary coded version is also regular and can be recognized by a 1DFA with at most n states, but at least 1+log(n) states. Here we shall present related results for two-way automata (2DFAs). First, we shall show that each unary 2DFA A' with n states can be converted to a 2DFA A'' recognizing bin(L(A')) with at most O(n.log n) states. If A' is minimal and uses only loops of odd lengths, A'' will use at most 2n+2 states, but it must use at least n states. For each n>=7, we shall also present a unary witness language for which a minimal 2DFA uses exactly n states, but any minimal 2DFA recognizing its binary coded version uses at least n states, but less than n+log(n) states.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.1}{10.4204/EPTCS.451.1}}

